X-ray Studies of Exoplanets: A 2020 Decadal Survey White Paper

Over the last two decades, the discovery of exoplanets has fundamentally changed our perception of the universe and humanity's place within it. Recent work indicates that a solar system's X-ray and high energy particle environment is of fundamental importance to the formation and development of the atmospheres of close-in planets such as hot Jupiters, and Earth-like planets around M stars. X-ray imaging and spectroscopy provide powerful and unique windows into the high energy flux that an exoplanet experiences, and X-ray photons also serve as proxies for potentially transfigurative coronal mass ejections. Finally, if the host star is a bright enough X-ray source, transit measurements akin to those in the optical and infrared are possible and allow for direct characterization of the upper atmospheres of exoplanets. In this brief white paper, we discuss contributions to the study of exoplanets and their environs which can be made by X-ray data of increasingly high quality that are achievable in the next 10--15 years.

==> Exo_refs.tex <==

\bibitem[Airapetian et al.(2016)]{Airapetian et al.(2016)} Airapetian, V.~S., Glocer, A., Gronoff, G., H{\'e}brard, E., \& Danchi, W.\ 2016, Nature Geoscience, 9, 452

\bibitem[Bhardwaj et al.(2007)]{Bhardwaj et al.(2007)} Bhardwaj, A., et 
al.\ 2007, Planetary and Space Science, 55, 1135

\bibitem[Cravens, Robertson, \& Snowden(2001)]{Cravens et al.(2001)} Cravens, T.~E., Robertson, I.~P., \& Snowden, S.~L.\ 2001, \jgr, 106, 24883 

\bibitem[Cuntz, Saar, \& Musielak(2000)]{Cuntz et al.(2000)} Cuntz, M., Saar, S.~H., \& Musielak, Z.~E.\ 2000, \apjl, 533, L151

\bibitem[Dong et al.(2018)]{Dong et al.(2018)} Dong, C.~F., Jin, M., Lingam, M., Airapetian, V. S., Ma, Y. J., van der Holst, B.\ 2018, Proc. Natl. Acad. Sci., 115, 260

\bibitem[Ehrenreich et al.(2015)]{Ehrenreich et al.(2015)} Ehrenreich, D., 
et al.\ 2015, \nat, 522, 459 

\bibitem[Erkaev et al.(2007)]{Erkaev et al.(2007)} Erkaev, N.~V., Kulikov, Y.~N., Lammer, H., Selsis, F., Langmayr, D., Jaritz, G.~F., \& Biernat, H.~K.\ 2007, \aap, 472, 329 

\bibitem[Fossati et al.(2010)]{Fossati et al.(2010)} Fossati, L., et al.\ 2010, \apjl, 714, L222 

\bibitem[Fulton \& Petigura(2018)]{Fulton et al.(2018)} Fulton, B.~J., \& Petigura, E.~A.\ 2018, \aj, 156, 264

\bibitem[Gillon et al.(2017)]{Gillon et al.(2017)} Gillon, M., et al.\ 2017, \nat, 542, 456 

\bibitem[Guedel(2007)]{Guedel(2007)} G{\"u}del, M.\ 2007, Living Reviews in Solar Physics, 4, 3 

\bibitem[Iro \& Deming(2010)]{Iro et al.(2010)} Iro, N., \& Deming, L.~D.\ 2010, \apj, 712, 218 

\bibitem[Kashyap, Drake, \& Saar(2008)]{Kashyap et al.(2008)} Kashyap, V.~L., Drake, J.~J., \& Saar, S.~H.\ 2008, \apj, 687, 

\bibitem[Kulow et al.(2014)]{Kulow et al.(2014)} Kulow, J.~R., France, K., Linsky, J., \& Loyd, R.~O.~P.\ 2014, \apj, 786, 132 

\bibitem[Lalitha, Schmitt, \& Dash(2018)]{Lalitha et al.(2018)} Lalitha, S., Schmitt, J.~H.~M.~M., \& Dash, S.\ 2018, \mnras, 477, 808 

\bibitem[Lammer et al.(2003)]{Lammer et al.(2003)} Lammer, H., Selsis, F., Ribas, I., Guinan, E.~F., Bauer, S.~J., \& Weiss, W.~W.\ 2003, \apjl, 598, L121 

\bibitem[Lanza(2009)]{Lanza(2009)} Lanza, A.~F.\ 2009, \aap, 505, 339 

\bibitem[Lanza(2012)]{Lanza(2012)} Lanza, A.~F.\ 2012, \aap, 544, A23 

\bibitem[Lavie et al.(2017)]{Lavie et al.(2017)} Lavie, B., et al.\ 2017,  \aap, 605, L7 

\bibitem[Lecavelier des Etangs et al.(2012)]{Lecavelier des Etangs et al.(2012)} Lecavelier des Etangs, A., et al.\ 2012, \aap, 543, L4 

\bibitem[Lingam et al.(2018)]{Lingam et al.(2018)} Lingam, M., Dong, C. F., Fang, X. H., Jakosky, B. M., Loeb, A.\ 2018, \apj, 853, 10 

\bibitem[Linsky et al.(2010)]{Linsky et al.(2010)} Linsky, J.~L., Yang, H., France, K., Froning, C.~S., Green, J.~C., Stocke, J.~T., \& Osterman, S.~N.\ 2010, \apj, 717, 1291 

\bibitem[Llama \& Shkolnik(2015)]{Llama et al.(2015)} Llama, J., \& Shkolnik, E.~L.\ 2015, \apj, 802, 41 
\bibitem[Lopez \& Fortney(2013)]{Lopez et al.(2013)} Lopez, E.~D., \& Fortney, J.~J.\ 2013, \apj, 776, 2 

\bibitem[Maggio et al.(2015)]{Maggio et al.(2015)} Maggio, A., et al.\ 2015, \apjl, 811, L2 

\bibitem[Miller et al.(2015)]{Miller et al.(2015)} Miller, B.~P., Gallo, E., Wright, J.~T., \& Pearson, E.~G.\ 2015, \apj, 799, 163 

\bibitem[Murray-Clay, Chiang, \& Murray(2009)]{Murray-Clay et al.(2009)} Murray-Clay, R.~A., Chiang, E.~I., \& Murray, N.\ 2009, \apj, 693, 23 

\bibitem[Owen \& Wu(2017)]{Owen et al.(2017)} Owen, J.~E., \& Wu, Y.\ 2017, \apj, 847, 29 

\bibitem[Owen \& Lai(2018)]{Owen et al.(2018)} Owen, J.~E., \& Lai, D.\ 2018, \mnras, 479, 5012 

\bibitem[Penz, Micela,  \& Lammer(2008)]{Penz et al.(2008)} Penz, T., Micela, G., \& Lammer, H.\ 2008, \aap, 477, 309 

\bibitem[Pillitteri et al.(2011)]{Pillitteri et al.(2011)} Pillitteri, I., G{\"u}nther, H.~M., Wolk, S.~J., Kashyap, V.~L., \& Cohen, O.\ 2011, \apjl, 741, L18 

\bibitem[Pillitteri et al.(2014)]{Pillitteri et al.(2014)} Pillitteri, I., Wolk, S.~J., Lopez-Santiago, J., G{\"u}nther, H.~M., Sciortino, S., Cohen, O., Kashyap, V., \& Drake, J.~J.\ 2014, \apj, 785, 145 

\bibitem[Poppenhaeger, Schmitt, \& Wolk(2013)]{Poppenhaeger et al.(2013)} Poppenhaeger, K., Schmitt, J.~H.~M.~M., \& Wolk, S.~J.\ 2013, \apj, 773, 62 

\bibitem[Poppenhaeger \& Wolk(2014)]{Poppenhaeger et al.(2014)} Poppenhaeger, K., \& Wolk, S.~J.\ 2014, \aap, 565, L1 

\bibitem[Sanz-Forcada et al.(2010)]{Sanz-Forcada et al.(2010)} Sanz-Forcada, J., Ribas, I., Micela, G., Pollock, A.~M.~T., Garc{\'{\i}}a-{\'A}lvarez, D., Solano, E., \& Eiroa, C.\ 2010, \aap, 511, L8 

\bibitem[Tian et al.(2005)]{Tian et al.(2005)} Tian, F., Toon, O.~B., Pavlov, A.~A., \& De Sterck, H.\ 2005, Science, 308, 1014 

\bibitem[Vidal-Madjar et al.(2003)]{Vidal-Madjar et al.(2003)} Vidal-Madjar, A., Lecavelier des Etangs, A., D{\'e}sert, J.-M., Ballester, G.~E., Ferlet, R., H{\'e}brard, G., \& Mayor, M.\ 2003, \nat, 422, 143

\bibitem[Wood et al.(2018)]{Wood et al.(2018)} Wood, B.~E., Laming, J.~M., Warren, H.~P., \& Poppenhaeger, K.\ 2018, \apj, 862, 66 

\bibitem[Yelle(2004)]{Yelle(2004)} Yelle, R.~V.\ 2004, \icarus, 170, 167 
